Scalable and Privacy-Preserving Federated Principal Component Analysis

Principal component analysis (PCA) is an essential algorithm for dimensionality reduction in many data science domains. We address the problem of performing a federated PCA on private data distributed among multiple data providers while ensuring data confidentiality. Our solution, SF-PCA, is an end-to-end secure system that preserves the confidentiality of both the original data and all intermediate results in a passive-adversary model with up to all-but-one colluding parties. SF-PCA jointly leverages multiparty homomorphic encryption, interactive protocols, and edge computing to efficiently interleave computations on local cleartext data with operations on collectively encrypted data. SF-PCA obtains results as accurate as non-secure centralized solutions, independently of the data distribution among the parties. It scales linearly or better with the dataset dimensions and with the number of data providers. SF-PCA is more precise than existing approaches that approximate the solution by combining local analysis results, and between 3x and 250x faster than privacy-preserving alternatives based solely on secure multiparty computation or homomorphic encryption. Our work demonstrates the practical applicability of secure and federated PCA on private distributed datasets.

==> figures/optimizations.tex <==
\section{Optimizations}

\subsection{Local Power Iterations}
https://arxiv.org/pdf/2002.08014.pdf

\subsection{Local Matrix Reduction}
http://www.cs.cmu.edu/~ninamf/papers/distributedPCAandCoresets.pdf

Liang et al. \vite{liang2014improved} relies on subspace embeddings such that nodes can locally reduce the size of their matrix before entering the collective algo.

\subsection{Cleartext Mean-Centralization}
